RGC: a radio AGN classifier based on deep learning. I. A semi-supervised multiclass model for VLA images

Bent radio active galactic nuclei (RAGNs) -- wide-angle tails (WATs) and narrow-angle tails (NATs) -- trace dense environments in galaxy groups and clusters, yet no multiclass classifier simultaneously separates them from straight Fanaroff--Riley types (sFRI, sFRII) using visually inspected labels and unlabelled data. We release FIRST-2060, a four-class labelled dataset of 2060 RAGNs (sFRI, sFRII, WAT, NAT) constructed from three publicly available catalogues through multi-tier visual inspection, together with the semi-supervised RGC 1.0 model that leverages 20,000 unlabelled sources. We benchmark RGC against five supervised baselines. FIRST-2060 is provided in two preprocessing variants: $\mathbf{R}_{L1}$, which retains spurious sources, and $\mathbf{R}_{L2}$, from which they are removed. The RGC model integrates the self-supervised framework BYOL (Bootstrap Your Own Latent) with an $E(2)$-equivariant steerable CNN (E2CNN) encoder, pre-trained on the unlabelled data and fine-tuned on the labelled sets. All six models are evaluated with 5-fold cross-validation, Grad-CAM attention analysis, and controlled class-imbalance experiments. ConvNeXT ($M_1$) and RGC ($M_2$) form a top tier at macro-$F_1$ $0.80\pm0.02$ and $0.79\pm0.02$ respectively, a difference within one standard deviation. $M_2$ is the only model whose Grad-CAM contours consistently trace the morphological structure of RAGNs -- lobes, jets, and bends -- rather than defaulting to compact blobs or diffuse patterns. The four-class scheme introduced here enables WAT/NAT-resolved catalogues that can serve as environment probes and progenitor classifications for diffuse cluster radio emission. The complementary strengths of $M_1$ and $M_2$ -- in cross-type and within-type discrimination respectively -- suggest that an ensemble approach may offer a practical framework for survey-scale morphological catalogues.

==> EXTRA.tex <==
In this section we will describe the Group Equivariant Convolutional Neural Netwrok, G-CNN in short. Recall that, traditional CNNs are only equivariant to translations, i.e., they are not invariant to rotations and reflections. A regular convolution operation is defined as:

$$(f \star \psi)(x) = \int f(y) \psi(x-y) dy$$
where $f$ is the input image, $\psi$ is the kernel, and $x$ is the location of the output pixel. This operation is translations equivariant, i.e., if we translate the input image by $t$ and apply the convolution operation, the output will be same as if we applied the convolution operation on the original image and then translated the output by $t$. We can easily see this as follows:

\begin{equation*}
    \begin{split}
    [[L_t(f)]\star \psi](x)&=\int L_t(f)(y) \psi(x-y) dy\\
     &=\int f(y-t) \psi(x-y) dy\\
     &=\int f(y) \psi(x-y+t) dy\\
     &=[L_t[f\star \psi ]](x)
    \end{split}
\end{equation*}
where $L_t$ is the translation operator. Hence, regular convolution and translation commute. That is
$$(L_t(f)\star \psi)(x) = L_t(f\star \psi)(x).$$
But, this is not true for rotation and reflection. For example, if we rotate the input image by $\theta$ and apply the convolution operation, the output will not be the same as if we applied the convolution operation on the original image and then rotated the output by $\theta$. We can see this by the following manipulations
\begin{equation*}
    \begin{split}
    [[R_\theta(f)]\star \psi](x)&=\int R_\theta(f)(y) \psi(x-y) dy\\
     &=\int f(R_\theta^{-1}(y)) \psi(x-y) dy\\
     &=\int f(R_{-\theta}(y)) \psi(x-y) dy\\
     &\neq \int f(y) \psi(R_\theta(x)-y) dy\\
     &=[R_\theta[f\star \psi ]](x)
    \end{split}
\end{equation*}
where $R_\theta$ is the rotation operator. From these computations, this is manifest that rotation and convolution do not commute. \\
\color{gray}
To make CNNs equivariant to rotations and reflections, G CNNs use group convolution instead of regular convolution, \cite{cohen16}. A group convolution is defined as:

$$(f \star \psi)(g) = \sum_{y \in \mathbb{Z}^2} f(y) \psi(g^{-1}y)$$

where $g$ is the group element, in the case of convolution, $g$ is the translation operator. The input image $f$ and the kernel $\psi$ are functions of the $\mathbb{Z}^2$ plane. The output of the convolution operation is a function on the discrete group $G$. As after the first convolution operation, the output is a function on the discrete group $G$, the subsequent convolution operations, the input image $f$ and the kernel $\psi$ are functions of the group $G$.

$$[f \star \psi](g) = \sum_{h \in G} f(h) \psi(h^{-1}g)$$

where $g$ is the group element, in the case of convolution. 

Now, with this definition of convolution, the rotation equivariance property still does not hold. To hold the Eucledian rotation equivariance property, the kernel $\psi$ must satisfy the following condition:

$$\psi(gx) = \rho_{out}(g)\psi(x)\rho_{in}(g)^{-1} \forall g \in G, x \in \mathbb{Z}^2$$

where $\rho$ is the representation of the group $G$. $\rho$ specifies how the channels of feature maps transform under the action of the group $G$. \\
\color{black}  
We want to generalize the idea of convolution for transformation under group operation. Recall that a group $G$ \cite{Rubakov2018} is a set of  elements with an operation defined on $G$ which maps $g_1, g_2 \in G$ to $g_1\cdot g_2=g_3 \in G$, and satisfies the following properties:
\begin{enumerate}
    \item For any three elements $g_1, g_2, g_3 \in G$, the following holds: $(g_1\cdot g_2)\cdot g_3= g_1 \cdot (g_2\cdot g_3)$.
    \item There exists an element $\mathbb{I}\in G $ such that for any $g\in G$, $g\cdot \mathbb{I}=\mathbb{I}\cdot g$. 
    \item  For all $g\in G$, there exists $g^{-1}\in G$ such that $g\cdot g^{-1}=g^{-1}\cdot g=\mathbb{I}$.
\end{enumerate}
Group equivariant convolution is defined as \cite{Cohen2016} 
\begin{equation}
    \left[ f\star \psi \right](g)=\sum_{y\in \mathbb{Z}^2} \sum_{k} f_k (y) \psi_k \left( g^{-1} y \right). \label{def1}
\end{equation}
Note that although the image $f(y)$ and $\psi(y)$ are functions on $\mathbb{Z}^2$, the convolution defined by Eq. \eqref{def1} is a function of $G$. After the first layer, the correlation function becomes 
\begin{equation}
    \left[ f\star g \right] (g)=\sum_{h\in G} \sum_k f_k (h) \psi_k \left( g^{-1} h \right). \label{def2} 
\end{equation}
From the definition \eqref{def2}, the equivariance under group operation is manifest which follows from the following manipulations
\begin{align}
   \left[[L_u f]\star \psi \right] (g)& =\sum_{h'\in G} \sum_k f_k (u^{-1}h') \psi_k \left( g^{-1} h' \right) , \\
   & =\sum_{h\in G} \sum_k f_k (h)\psi (g^{-1} u h), \\
   &= \sum_{h\in G} \sum_k f_k (h) f_k (h) \psi \left( (u^{-1} g)^{-1}h \right), \\
   &= \left[ L_u \left[f\star \psi \right] \right] (g), 
\end{align}
where going from the first to second line we have used the redefinition $u^{-1}h'=h$. \\
In this work, we  used CNN which are equivariant under the Eucildean group SE$(2)$, which is defined as the group of isometries of $\mathbb{R}^2$, and continuously connected to the identity. In other words, the group under consideration is the direct product of rotation group SO$(2)$ and translation $P_i$, i.e. $G=\text{SO}(2)\otimes P_i $. 
% \subsection{Data augmentation}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Train-Val-Accuracy.pdf}
%     \caption{Caption}
%     \label{fig:accuracy}
% \end{figure}
